Improving Opinion-based Question Answering Systems Through Label Error Detection and Overwrite

Label error is a ubiquitous problem in annotated data. Large amounts of label error substantially degrades the quality of deep learning models. Existing methods to tackle the label error problem largely focus on the classification task, and either rely on task specific architecture or require non-trivial additional computations, which is undesirable or even unattainable for industry usage. In this paper, we propose LEDO: a model-agnostic and computationally efficient framework for Label Error Detection and Overwrite. LEDO is based on Monte Carlo Dropout combined with uncertainty metrics, and can be easily generalized to multiple tasks and data sets. Applying LEDO to an industry opinion-based question answering system demonstrates it is effective at improving accuracy in all the core models. Specifically, LEDO brings 1.1% MRR gain for the retrieval model, 1.5% PR AUC improvement for the machine reading comprehension model, and 0.9% rise in the Average Precision for the ranker, on top of the strong baselines with a large-scale social media dataset. Importantly, LEDO is computationally efficient compared to methods that require loss function change, and cost-effective as the resulting data can be used in the same continuous training pipeline for production. Further analysis shows that these gains come from an improved decision boundary after cleaning the label errors existed in the training data.

==> achknowledgement.tex <==
\section*{Acknowledgements}


==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Many strategies have been proposed to tackle the label error (or \textit{noisy label}) problem. However, most of the existing methods focus on classification tasks \cite{song2022learning}. In contrast, LEDO is model-agnostic, and can generalize to other supervised tasks such as retrieval and ranking.  

Song et al. categorized existing methods into 5 major groups: \textit{robust architecture}, \textit{robust regularization}, \textit{robust loss function}, \textit{loss adjustment}, and \textit{sample selection} \cite{song2022learning}. According to this categorization, LEDO falls into the \textit{sample selection} category. Sample selection methods generally reply on the \textit{small-loss} trick, which assumes true-labeled examples tend to have small loss based on the finding that deep learning models usually learn from easy and clean examples first, and then memorizes hard or error examples in later learning stage \cite{arpit2017closer}. Both MentorNet \cite{jiang2018mentornet} and Co-teaching \cite{han2018co} are built upon this assumption, and uses a teacher model (in MentorNet) or a peer model (in Co-teaching) to select a subset of ``clean" examples to train the target model at each iteration. However, the \textit{small-loss} trick does not work well for the \textit{asymmetric noise} (where a class is more likely to be mis-labeled as some particular classes rather than equally to all other classes) \cite{song2022learning}. 

Besides multi-network learning, researchers also tried multi-round learning to iteratively refine the training data to identify the clean subset. INCV \cite{chen2019understanding} uses cross-validation to identify examples with label error and also removes large loss examples iteratively to reduce the error rate from the original data, then applies Co-teaching on the reduced error data. It requires the model prediction to agree with the label to indicate the label is ``correct", which is a strict criteria. SELF \cite{nguyen2019self} takes a hybrid approach which first uses a mean-teacher \cite{tarvainen2017mean} to filter out error examples in the supervised loss, then applies semi-supervised loss on the filtered examples. Both INCV and SELF are designed and tested only for classification tasks. 

Different from the existing approaches, LEDO involves \textit{sentinel models} in a more flexible manner to provide signals about whether a label is correct. It also brings in external information when a separate sentinel model (different from the target model) is used. Besides, by introducing the \textit{uncertainty metrics}, it provides control knobs to mitigate the over-correction or under-correction problems. 

